First observation of isolated nuclear recoils following neutron capture for dark matter calibration

Low-energy nuclear recoils (NRs) are hard to measure because they produce few e$^{-}$/h$^+$ pairs in solids -- i.e. they have low "ionization yield". A silicon detector was exposed to thermal neutrons over 2.5\,live-days, probing NRs down to 450\,eV. The observation of a neutron capture-induced component of NRs at low energies is supported by the much-improved fit upon inclusion of a capture NR model. This result shows that thermal neutron calibration of very low recoil energy NRs is promising for dark matter searches, coherent neutrino experiments, and improving understanding of ionization dynamics in solids.

==> Makefile <==
# input files
file = thermaln_prd_arxiv  
texfile = $(shell find . -type f -name '*.tex')
imgpng = $(shell find . -type f -name '*.png')
imgeps = $(shell find . -type f -name '*.eps')
imgpdf = $(patsubst %.eps, %.pdf, $(imgeps))

#all: $(file).pdf 

$(file).pdf: $(texfile) $(wildcard *.bib) $(imgpdf) $(imgpng)
	pdflatex $(file)
	bibtex $(file)
	pdflatex $(file)
	pdflatex $(file)

# convert eps image to pdf
$(imgpdf): %.pdf: %.eps
	ps2pdf  -dEPSCrop  $< $@

clean:
	find . \( -name '*.aux' -o -name '*.log' -o -name '*~' -o -name '*.blg' -o -name '*.bbl' \) -exec rm '{}' \;
	rm $(imgpdf)

test:
	@echo $(imgeps)
	@echo $(imgpdf)



==> authorinst.tex <==
\affiliation{Department of Physics, University of Colorado Denver, Denver, Colorado 80217, USA} 
\affiliation{School of Physics \& Astronomy, University of Minnesota, Minneapolis, Minnesota 55455, USA}

